Comparison of Machine Learning Approaches for Classifying Spinodal Events

In this work, we compare the performance of deep learning models for classifying the spinodal dataset. We evaluate state-of-the-art models (MobileViT, NAT, EfficientNet, CNN), alongside several ensemble models (majority voting, AdaBoost). Additionally, we explore the dataset in a transformed color space. Our findings show that NAT and MobileViT outperform other models, achieving the highest metrics-accuracy, AUC, and F1 score on both training and testing data (NAT: 94.65, 0.98, 0.94; MobileViT: 94.20, 0.98, 0.94), surpassing the earlier CNN model (88.44, 0.95, 0.88). We also discuss failure cases for the top performing models.

==> REFDATA.tex <==

The architecture of the reference CNN from \cite{Benato_2022} is shown in Fig. \ref{fig1}. It begins with an input layer that performs a 2D convolution using 15 filters, each of size 3x3. These filters scan small patches of the input image with a stride of 1. The activation function used is ReLU, which introduces non-linearity by zeroing out negative values. Following the first convolution layer, there is a max pooling layer with a 2x2 window, which reduces the spatial dimensions, helping the network to focus on important features while reducing computational complexity. 
 \begin{figure}[h]
  \centering
  \includegraphics[scale=0.4]{Figures/Architechture.png}   
  \captionsetup{justification=raggedright, singlelinecheck=false}
  \caption{Architecture diagram of the Reference CNN network.}

  \label{fig1}
\end{figure}
Next, a second convolution layer, similar to the first, is added to learn more detailed features. After the second pooling layer, a third convolution layer with 25 filters is applied to extract even more complex patterns. Following the convolution layers, a dropout layer with a rate of 0.4 is introduced to prevent overfitting. After the dropout, the model includes a flattening step, followed by a dense layer with 10 neurons and ReLU activation. This dense layer consolidates the features extracted by the convolution layers into a more interpretable form for classification.


The final output is produced by a single neuron with a sigmoid activation function, providing the model's prediction as a probability for the two classes.







